Dynamical inverse seesaw mechanism as a simple benchmark for electroweak breaking and Higgs boson studies

The Standard Model(SM) vacuum is unstable for the measured values of the top Yukawa coupling and Higgs mass. Here we study the issue of vacuum stability when neutrino masses are generated through spontaneous low-scale lepton number violation. In the simplest dynamical inverse seesaw, the SM Higgs has two siblings: a massive CP-even scalar plus a massless Nambu-Goldstone boson, called majoron. For TeV scale breaking of lepton number, Higgs bosons can have a sizeable decay into the invisible majorons. We examine the interplay and complementarity of vacuum stability and perturbativity restrictions, with collider constraints on visible and invisible Higgs boson decay channels. This simple framework may help guiding further studies, for example, at the proposed FCC facility.

==> Makefile <==
FILENAME=invisible-15feb
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = invisible-15feb.ps 
PDFFILE = invisible-15feb.pdf

COPY = if test -r invisible-15feb.toc; then cp invisible-15feb.toc invisible-15feb.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f invisible-15feb.aux invisible-15feb.log invisible-15feb.dvi invisible-15feb.toc invisible-15feb.out invisible-15feb.blg invisible-15feb.mtc invisible-15feb.mtc1 invisible-15feb.rel invisible-15feb.vrb invisible-15feb.end invisible-15feb.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" invisible-15feb.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	invisible-15feb.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	PhysBiblio.exe tex bibliography.bib './invisible-15feb.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


